MCoNaLa: A Benchmark for Code Generation from Multiple Natural Languages

While there has been a recent burgeoning of applications at the intersection of natural and programming languages, such as code generation and code summarization, these applications are usually English-centric. This creates a barrier for program developers who are not proficient in English. To mitigate this gap in technology development across languages, we propose a multilingual dataset, MCoNaLa, to benchmark code generation from natural language commands extending beyond English. Modeled off of the methodology from the English Code/Natural Language Challenge (CoNaLa) dataset, we annotated a total of 896 NL-code pairs in three languages: Spanish, Japanese, and Russian. We present a quantitative evaluation of performance on the MCoNaLa dataset by testing with state-of-the-art code generation systems. While the difficulties vary across these three languages, all systems lag significantly behind their English counterparts, revealing the challenges in adapting code generation to new languages.

==> sections/app1_quality_of_auto-translation.tex <==
\section{Quality of Auto-translation}
\label{app1:translation}

\begin{figure*}[h]
    \centering
    \includegraphics[width=15.4cm]{./pic/translation-quality.pdf}
    \caption{Examples showing that the translation errors or omits critical words in the original intent. }
    \label{fig:translation-semantic}
\end{figure*}

To have an intuitive grasp on the quality of translated NL intents, we perform a manual check with the assistance of the Google Translate API and dictionaries, particularly in the degree of semantic alignment between the \textsc{M2M-124} translated intents and the original ones (in the context of the paired code snippet). 
Concretely, we randomly select 20 CoNaLa samples and check if the semantic is preserved after translating the intents from English into three target languages (\textit{translate-train}). Similarly, we also sample 20 cases from MCoNaLa in each target language subset and compare with the translated English intents (\textit{translate-test}). 

% Our analysis notices two major problems brought by the intent translation process. 

As shown in~\autoref{fig:translation-semantic}, translations of the MMT model are still rather sub-optimal. It often translates the important words incorrectly, sometimes even omitting these words. This loss is especially severe on verbs that strongly indicate certain Python operations. As a result, the translation process may impair the alignment between intents and snippets, being one of the major factors to the poor performance in translated settings. 

==> sections/app3_significance_test.tex <==
\section{Significance Test}
\label{app3:significance-test}

To support the effectiveness of our data benchmark, we perform significance tests to demonstrate that every language subset of MCoNaLa is informative of showing significant differences between systems. 
According to the baseline experiments discussed in~\autoref{subsec:method-model}, we conduct significance test on each pair of baseline models. More specifically, we use paired bootstrap re-sampling method, with a sample rate of $0.5$ and a sample size of $10,000$ on each setting and each language subset. 

\begin{table}[H]
\centering
\resizebox{0.49\textwidth}{!}{
    \begin{tabular}{cc|ccc|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Setting}} & \multirow{2}{*}{\textbf{Language}} & \multicolumn{3}{c|}{\textbf{Win Rate (\%)}} & \multirow{2}{*}{\textbf{Tie}} & \multirow{2}{*}{\textbf{p-value}} \\
    \cmidrule{3-5}
    {} & {} & \textbf{\textsc{mBART}} & \textbf{\textsc{TranX}} & \textbf{\textsc{TAE}} & {} & {} \\ 
    \midrule
    \multirow{9}{*}{translate-test} & \multirow{3}{*}{es} & {0.532} & {0.402} & {-} & {0.066} & {0.468} \\
    {} & {} & {0.522} & {-} & {0.396} & {0.102} & {0.478} \\
    {} & {} & {-} & {0.508} & {0.448} & {0.044} & {0.492} \\
    \cmidrule{2-7}
    {} & \multirow{3}{*}{ja} & {0.000} & {1.000} & {-} & {0.000} & {0.000} \\
    {} & {} & {0.000} & {-} & {1.000} & {0.000} & {0.000} \\
    {} & {} & {-} & {0.002} & {0.998} & {0.000} & {0.002} \\
    \cmidrule{2-7}
    {} & \multirow{3}{*}{ru} & {0.000} & {1.000} & {-} & {0.000} & {0.000} \\
    {} & {} & {0.000} & {-} & {1.000} & {0.000} & {0.000} \\
    {} & {} & {-} & {0.001} & {0.998} & {0.001} & {0.002} \\
    \midrule
    \multirow{3}{*}{translate-train} & {es} & {0.592} & {0.408} & {-} & {0.000} & {0.408} \\
    \cmidrule{2-7}
    {} & {ja} & {0.000} & {1.000} & {-} & {0.000} & {0.000} \\
    \cmidrule{2-7}
    {} & {ru} & {0.000} & {1.000} & {-} & {0.000} & {0.000} \\
    \bottomrule
    \end{tabular}
}
\caption{Significance testing results between each pair of baseline models. `-' marks the model not in the pair.} 
\label{tab:sig-test-model}
\end{table}

As shown in~\autoref{tab:sig-test-model}, in both \textit{translate-test} and \textit{translate-train} settings, code-specific systems (i.e., \textsc{TranX} and \textsc{TAE}) significantly outperform \textsc{mBART} on Japanese and Russian subsets. For Spanish, as expected given its relative difficulty, there are no significant differences between systems. 

The above tests demonstrate the usage of significance testing~\citep{dror2018hitchhiker} to determine the reliability of results, even on a relatively small dataset. While small datasets are not entirely desirable for informative evaluation, the resulting sizes of datasets are practical reflections of the data availability and collection difficulty for each language, supporting our call for more resource developments for non-English languages.
